Lamb modes and Born approximation for small shape defects inversion in elastic plates

The aim of this work is to present theoretical tools to study wave propagation in elastic waveguides and perform multi-frequency scattering inversion to reconstruct small shape defects in a 2D and 3D elastic plate. Given surface multi-frequency wavefield measurements, we use a Born approximation to reconstruct localized defect in the geometry of the plate. To justify this approximation, we introduce a rigorous framework to study the propagation of elastic wavefield generated by arbitrary sources. By studying the decreasing rate of the series of inhomogeneous Lamb mode, we prove the well-posedness of the PDE that model elastic wave propagation in 2D and 3D planar waveguides. We also characterize the critical frequencies for which the Lamb decomposition is not valid. Using these results, we generalize the shape reconstruction method already developed for acoustic waveguide to 2D elastic waveguides and provide a stable reconstruction method based on a mode-by-mode spacial Fourier inversion given by the scattered field.

==> [4] Elastic problem in regular waveguides/disp3D.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.49412,0.18431,0.55686}%
\definecolor{mycolor2}{rgb}{0.92941,0.69412,0.12549}%
\definecolor{mycolor3}{rgb}{0.46667,0.67451,0.18824}%
%
\begin{tikzpicture}

\begin{axis}[%
width=3.5in,
height=2in,
at={(0in,0in)},
scale only axis,
xmin=0,
xmax=9,
tick align=outside,
xlabel style={font=\color{white!15!black}},
xlabel={$\text{Imag}(k)h$},
ymin=0,
ymax=9,
ylabel style={font=\color{white!15!black}},
ylabel={$\text{Real}(k)h$},
zmin=0,
zmax=4.5,
zlabel style={font=\color{white!15!black}},
zlabel={$\omega h$},
view={138.3}{15},
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left,
axis z line*=left,
xmajorgrids,
ymajorgrids,
zmajorgrids,
legend columns=4,
legend style={at={(0in,-1in)}, anchor=north, legend cell align=left, align=left, draw=white!15!black}
]
\addplot3 [color=mycolor1]
 table[row sep=crcr] {%
0	0	0\\
0	0.240883506007369	0.2\\
0	0.516429946808469	0.426315789473684\\
0	0.800996083737869	0.652631578947368\\
0	1.1130476512379	0.878947368421052\\
0	1.55552956026594	1.10526315789474\\
0	2.19740974882412	1.29\\
0	2.23331129543969	1.3\\
0	2.26885934964659	1.31\\
0	2.30404198126399	1.32\\
0	2.33885314434443	1.33\\
0	2.34431553880598	1.33157894736842\\
0	2.57236421211736	1.4\\
0	2.63604966198043	1.42\\
0	2.69853589668749	1.44\\
0	2.75990658274721	1.46\\
0	2.82024184688878	1.48\\
0	2.87961699215255	1.5\\
0	2.93810196671468	1.52\\
0	2.9957612757504	1.54\\
0	3.04669986176604	1.5578947368421\\
0	3.05265414463145	1.56\\
0	3.10883481588893	1.58\\
0	3.65129722375212	1.78421052631579\\
0	4.20999045519639	2.01052631578947\\
0	4.74400350447294	2.23684210526316\\
0	5.26339293412722	2.46315789473684\\
0	5.77355476854468	2.68947368421053\\
0	6.27764061284368	2.91578947368421\\
0	6.68483534234022	3.1\\
0	6.72156862045414	3.11666666666667\\
0	6.75828596212113	3.13333333333333\\
0	6.77760461855843	3.14210526315789\\
0	6.7949877822824	3.15\\
0	6.83167448386764	3.16666666666667\\
0	6.86834645819949	3.18333333333333\\
0	6.90500408538187	3.2\\
0	7.27471249916745	3.36842105263158\\
0	7.76981113949281	3.59473684210526\\
0	8.26348115352777	3.82105263157895\\
0	8.75612789121009	4.04736842105263\\
0	8.97928085544083	4.15\\
0	9.01550662974932	4.16666666666667\\
0	9.05172907115394	4.18333333333333\\
0	9.08794825859402	4.2\\
0	9.12416426910582	4.21666666666667\\
0	9.16037717787087	4.23333333333333\\
0	9.1965870582628	4.25\\
0	9.24803813473117	4.27368421052632\\
0	9.73941671928904	4.5\\
};
 \addlegendentry{propagative}
 
 \addplot3 [color=mycolor2]
 table[row sep=crcr] {%
2.1	1.1	0\\
2.07866245105832	1.12781655692737	0.2\\
1.97800055667293	1.13585009470251	0.426315789473684\\
1.79143748136056	1.14659298378768	0.652631578947368\\
1.48832007640335	1.15007254679957	0.878947368421052\\
0.993934770231269	1.09252013560374	1.10526315789474\\
0.377109202658498	0.900886853154025	1.29\\
0.321118047925784	0.889245670224501	1.3\\
0.252980509367854	0.87759990018768	1.31\\
0.157260113931674	0.865913648710013	1.32\\
0	0.86	1.33\\
};
 \addlegendentry{inhomogeneous}
 
 \addplot3 [color=mycolor3]
 table[row sep=crcr] {%
0	0	1.41\\
0.110348657321558	1.97367332576898e-32	1.42\\
0.202993539038354	4.75962381000363e-20	1.44\\
0.240527958062569	1.92706163283939e-17	1.46\\
0.253676788860733	9.26526018054846e-20	1.48\\
0.249493455574741	3.4411734240258e-19	1.5\\
0.229485146994256	2.10834442000559e-19	1.52\\
0.190919391332875	7.94513913458266e-30	1.54\\
0.129871976357745	5.10176195536929e-18	1.5578947368421\\
0.119444751023683	1.30309058449776e-18	1.56\\
0	0	1.57\\
};
 \addlegendentry{evanescent}


\addplot3 [color=red, draw=none, mark size=3pt, mark=*, mark options={solid, red}]
 table[row sep=crcr] {%
0	0.86	1.33\\
};
 \addlegendentry{critical}
 
\addplot3 [color=mycolor1]
 table[row sep=crcr] {%
0	0.86	1.33\\
0	0.97590831019793	1.33\\
0	0.99756136683486	1.33157894736842\\
0	1.32447804248352	1.4\\
0	1.37632788953081	1.42\\
0	1.42235237917737	1.44\\
0	1.46428199283637	1.46\\
0	1.50319320637873	1.48\\
0	1.53980232711123	1.5\\
0	1.57460970143863	1.52\\
0	1.60797794914228	1.54\\
0	1.6368366577503	1.5578947368421\\
0	1.6401776455397	1.56\\
0	1.67141554211096	1.58\\
0	1.96038521534047	1.78421052631579\\
0	2.25683913369543	2.01052631578947\\
0	2.55171530047755	2.23684210526316\\
0	2.85991020320321	2.46315789473684\\
0	3.20581457348159	2.68947368421053\\
0	3.63630179927183	2.91578947368421\\
0	4.07654009979244	3.1\\
0	4.1199530081647	3.11666666666667\\
0	4.16384061819158	3.13333333333333\\
0	4.18711890040371	3.14210526315789\\
0	4.20816996583333	3.15\\
0	4.25290768578687	3.16666666666667\\
0	4.29802035439543	3.18333333333333\\
0	4.3434748005336	3.2\\
0	4.81512006902359	3.36842105263158\\
0	5.45531087783131	3.59473684210526\\
0	6.07840031088174	3.82105263157895\\
0	6.6785035831606	4.04736842105263\\
0	6.94344053467028	4.15\\
0	6.98607080116032	4.16666666666667\\
0	7.0285947746092	4.18333333333333\\
0	7.07101382995078	4.2\\
0	7.11332934200008	4.21666666666667\\
0	7.15554268333149	4.23333333333333\\
0	7.19765522237926	4.25\\
0	7.2573286260121	4.27368421052632\\
0	7.8181494408948	4.5\\
};

\addplot3 [color=mycolor1]
 table[row sep=crcr] {%
0	0.86	1.33\\
0	0.732360062616439	1.33\\
0	0.706960975895301	1.33157894736842\\
0	0.180806227936437	1.4\\
0	0	1.41\\
};


\addplot3 [color=mycolor1]
 table[row sep=crcr] {%
0	0	1.57\\
0	0.115591704166184	1.58\\
0	0.733022796465536	1.78421052631579\\
0	1.22848725945342	2.01052631578947\\
0	1.68182902360143	2.23684210526316\\
0	2.12014218120227	2.46315789473684\\
0	2.55254326677792	2.68947368421053\\
0	2.96551493324672	2.91578947368421\\
0	3.26767623023752	3.1\\
0	3.29333338543879	3.11666666666667\\
0	3.31873804224581	3.13333333333333\\
0	3.33201059555273	3.14210526315789\\
0	3.34389942049374	3.15\\
0	3.36882715284669	3.16666666666667\\
0	3.39353114931094	3.18333333333333\\
0	3.41802147695046	3.2\\
0	3.65573645686971	3.36842105263158\\
0	3.95802406645645	3.59473684210526\\
0	4.25408055751335	3.82105263157895\\
0	4.5551551754052	4.04736842105263\\
0	4.69685407049827	4.15\\
0	4.72034251293643	4.16666666666667\\
0	4.74398829920397	4.18333333333333\\
0	4.76780114154272	4.2\\
0	4.79179117276012	4.21666666666667\\
0	4.81596895150951	4.23333333333333\\
0	4.84034546397289	4.25\\
0	4.875350108547	4.27368421052632\\
0	5.23843141872546	4.5\\
};

\addplot3 [color=mycolor1]
 table[row sep=crcr] {%
0	0	3.14\\
0	0.13160065995674	3.14210526315789\\
0	0.525939470925294	3.15\\
0	0.886378440678038	3.16666666666667\\
0	1.12004328931699	3.18333333333333\\
0	1.30093214057127	3.2\\
0	2.2802088420898	3.36842105263158\\
0	2.96964778766511	3.59473684210526\\
0	3.47433208461264	3.82105263157895\\
0	3.9107035429219	4.04736842105263\\
0	4.09696380650802	4.15\\
0	4.12670961720399	4.16666666666667\\
0	4.15632541280098	4.18333333333333\\
0	4.18581356756596	4.2\\
0	4.21517589039606	4.21666666666667\\
0	4.24441363740178	4.23333333333333\\
0	4.27352752558283	4.25\\
0	4.31468710249938	4.27368421052632\\
0	4.69447735608529	4.5\\
};

\addplot3 [color=mycolor3]
 table[row sep=crcr] {%
1.67	0	3.09\\
1.32765705101711	3.3538423211248e-19	3.1\\
0.969718842644492	7.8278431438213e-18	3.11666666666667\\
0.53701449483885	7.53607843318965e-36	3.13333333333333\\
0	0	3.14\\
};

\addplot3 [color=mycolor3]
 table[row sep=crcr] {%
1.67	0	3.09\\
2.16513252258002	2.66298700450358e-18	3.1\\
2.27529924060965	3.96031708456293e-16	3.11666666666667\\
2.34479925812492	4.39215613719778e-17	3.13333333333333\\
2.37286801230704	1.8054227205837e-29	3.14210526315789\\
2.39464484040097	5.52679595341827e-18	3.15\\
2.43240372660125	5.07898230578781e-19	3.16666666666667\\
2.46179517924899	1.62409972150637e-18	3.18333333333333\\
2.4849594927319	3.58225419530341e-18	3.2\\
2.54319124546004	2.23666095260622e-16	3.36842105263158\\
2.39039551798377	1.62173839979295e-18	3.59473684210526\\
2.06520460608611	3.00410058465913e-18	3.82105263157895\\
1.50086603815476	5.75296301559461e-18	4.04736842105263\\
1.06457496844018	1.28994904135939e-16	4.15\\
0.967913759582484	7.1275958386418e-32	4.16666666666667\\
0.857804226193199	1.65297874902769e-23	4.18333333333333\\
0.728029797684183	9.23639222435766e-22	4.2\\
0.565005700427919	1.66102109133121e-17	4.21666666666667\\
0.321244724940165	1.99254213958763e-17	4.23333333333333\\
0	0	4.24\\
};

\addplot3 [color=mycolor1]
 table[row sep=crcr] {%
0	0	4.24\\
0	0.34399651910184	4.25\\
0	0.665698756435447	4.27368421052632\\
0	2.07891596865504	4.5\\
};

\addplot3 [color=mycolor2]
 table[row sep=crcr] {%
5.35	1.55	0\\
5.34636585203204	1.55248619959508	0.2\\
5.31111874657124	1.55562309038836	0.426315789473684\\
5.24982048536024	1.56067459146211	0.652631578947368\\
5.16150622636096	1.56704886263138	0.878947368421052\\
5.04470671615407	1.57383049065776	1.10526315789474\\
4.92681338918179	1.57874774611822	1.29\\
4.91982259445559	1.57897774313947	1.3\\
4.91276745435167	1.5792028112157	1.31\\
4.90564768595054	1.57942275536713	1.32\\
4.89846300219128	1.57963737709367	1.33\\
4.89732262525608	1.57967076495916	1.33157894736842\\
4.84632757320538	1.58097325068134	1.4\\
4.8308301584968	1.58129486339093	1.42\\
4.81506062552656	1.58158639352655	1.44\\
4.79901625737324	1.58184587871122	1.46\\
4.78269425587838	1.58207128060521	1.48\\
4.76609173895669	1.58226048114528	1.5\\
4.74920573778894	1.58241127854534	1.52\\
4.73203319389211	1.58252138304174	1.54\\
4.71642282422742	1.58258345804153	1.5578947368421\\
4.71457095606096	1.58258841236464	1.56\\
4.69681577717499	1.58260988691552	1.58\\
4.49792223892842	1.57955695843112	1.78421052631579\\
4.23606219617969	1.56578532417173	2.01052631578947\\
3.92255724717724	1.53304523398935	2.23684210526316\\
3.54513026165767	1.46596178268117	2.46315789473684\\
3.08427572489323	1.3320252851266	2.68947368421053\\
2.49674488427738	1.0386493910161	2.91578947368421\\
2	0.5	3\\
1.67	0	3.09\\
};

\addplot3 [color=mycolor3]
 table[row sep=crcr] {%
5.13	0	4.13\\
4.90661720049872	6.56886885060537e-18	4.15\\
4.67460889148372	3.24556372808638e-22	4.16666666666667\\
4.50907290425882	1.83944069766621e-18	4.18333333333333\\
4.36585832645494	2.91208098923321e-15	4.2\\
4.23450769635484	2.53397792572304e-18	4.21666666666667\\
4.11052967311173	3.37887369973242e-19	4.23333333333333\\
3.99150460477086	1.31243513389077e-18	4.25\\
3.82808492811461	2.19443255553788e-18	4.27368421052632\\
2.33644018864079	2.54648435351496e-17	4.5\\
};

\addplot3 [color=mycolor3]
 table[row sep=crcr] {%
5.13	0	4.13\\
5.25420903629714	3.01222391780279e-17	4.15\\
5.4063637273704	1.01981867710077e-17	4.16666666666667\\
5.49099763654835	9.30292462113608e-19	4.18333333333333\\
5.5522418219749	5.01307568369757e-16	4.2\\
5.60053402687898	1.68983754188987e-18	4.21666666666667\\
5.64034607080131	1.76001077607364e-18	4.23333333333333\\
5.67407832270764	2.10178530370005e-18	4.25\\
5.71431670256205	6.86944902763401e-17	4.27368421052632\\
5.89814965266592	1.53992957482988e-16	4.5\\
};

\addplot3 [color=mycolor2]
 table[row sep=crcr] {%
8.55	1.77	0\\
8.53053533711119	1.77604117754819	0.2\\
8.50871003381698	1.77775967261154	0.426315789473684\\
8.47095589978058	1.78055606215709	0.652631578947368\\
8.41702004261158	1.78416373558135	0.878947368421052\\
8.34653336573854	1.78819181631449	1.10526315789474\\
8.27638605118873	1.79142694642793	1.29\\
8.27225854748191	1.79159321012977	1.3\\
8.26809672518404	1.79175814055681	1.31\\
8.26390052383507	1.79192167175562	1.32\\
8.25966988234241	1.7920837370163	1.33\\
8.25899873399921	1.79210918783658	1.33157894736842\\
8.22908580102732	1.79317138131517	1.4\\
8.22003390280957	1.79346496499292	1.42\\
8.21084165613514	1.79374984188381	1.44\\
8.20150851116873	1.79402540374887	1.46\\
8.1920339068697	1.79429102836547	1.48\\
8.1824172708055	1.79454607919231	1.5\\
8.17265801895946	1.79478990502075	1.52\\
8.16275555553253	1.79502183961174	1.54\\
8.15377356718636	1.79521872329856	1.5578947368421\\
8.15270927273902	1.79524120131784	1.56\\
8.14251855059598	1.79544729268961	1.58\\
8.03004495686103	1.79661651493749	1.78421052631579\\
7.88679448417014	1.79512756858609	2.01052631578947\\
7.72274846829983	1.78920339891138	2.23684210526316\\
7.53630699090264	1.77675537352418	2.46315789473684\\
7.32544098148067	1.7548739314791	2.68947368421053\\
7.0875395077285	1.71933140453899	2.91578947368421\\
6.87160214387168	1.67593540268143	3.1\\
6.85099271426963	1.67118754313136	3.11666666666667\\
6.83019704003714	1.66628382963998	3.13333333333333\\
6.81917644213118	1.66363859086504	3.14210526315789\\
6.80921304933123	1.66121910268774	3.15\\
6.78803862043577	1.65598797824029	3.16666666666667\\
6.76667158016639	1.6505848344802	3.18333333333333\\
6.74510970221266	1.64500379753353	3.2\\
6.51574144502995	1.57707085330183	3.36842105263158\\
6.17083478974407	1.43988831295128	3.59473684210526\\
5.77524894362692	1.20850869829251	3.82105263157895\\
5.31531915871317	0.733623291479004	4.04736842105263\\
5.13	0	4.13\\
};

\addplot3 [color=mycolor2]
 table[row sep=crcr] {%
9.88950096731688	1.75980149640599	3.82105263157895\\
9.63633122578271	1.67446484002985	4.04736842105263\\
9.51309141337675	1.62461117565365	4.15\\
9.49254051156653	1.61570107886133	4.16666666666667\\
9.47183399851277	1.60654132996533	4.18333333333333\\
9.45096971408258	1.59712277325118	4.2\\
9.4299454121101	1.58743574353981	4.21666666666667\\
9.40875875475358	1.57747002587682	4.23333333333333\\
9.38740730634489	1.56721481102705	4.25\\
9.35677729133344	1.55212100252853	4.27368421052632\\
9.04530520612507	1.36871062225569	4.5\\
};


\addplot3 [color=red, draw=none, mark size=3.0pt, mark=*, mark options={solid, red}]
 table[row sep=crcr] {%
0	0	1.41\\
};

\addplot3 [color=red, draw=none, mark size=3.0pt, mark=*, mark options={solid, red}]
 table[row sep=crcr] {%
0	0	1.57\\
};

\addplot3 [color=red, draw=none, mark size=3.0pt, mark=*, mark options={solid, red}]
 table[row sep=crcr] {%
0	0	3.14\\
};

\addplot3 [color=red, draw=none, mark size=3.0pt, mark=*, mark options={solid, red}]
 table[row sep=crcr] {%
0	0	4.24\\
};


\addplot3 [color=red, draw=none, mark size=3.0pt, mark=*, mark options={solid, red}]
 table[row sep=crcr] {%
1.67	0	3.09\\
};


\addplot3 [color=red, draw=none, mark size=3.0pt, mark=*, mark options={solid, red}]
 table[row sep=crcr] {%
5.13	0	4.13\\
};


\end{axis}
\end{tikzpicture}%

==> [4] Elastic problem in regular waveguides/rcmode.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
%
\begin{tikzpicture}

\begin{axis}[%
width=3.3in,
grid=major,
height=1.2in,
at={(0in,0in)},
scale only axis,
xlabel={$\Real(k)$}, 
ylabel={$\Imag(k)$},
xmin=-4,
xmax=4,
ymin=-15,
ymax=15,
axis background/.style={fill=white},
legend style={at={(3.4in,1.2in)},anchor=north west, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1, draw=none, mark=o, mark options={solid, mycolor1}]
  table[row sep=crcr]{%
1.4206909912883	3.00282300676693\\
-1.4206909912883	3.00282300676693\\
1.58043854208169	4.86906922382785\\
-1.58043854208169	4.86906922382785\\
1.69801972355383	6.58397118804595\\
-1.69801972355383	6.58397118804595\\
1.79271597755113	8.24240167067542\\
-1.79271597755113	8.24240167067542\\
1.872244836012	9.8727432041414\\
-1.872244836012	9.8727432041414\\
1.94086340252889	11.486876054131\\
-1.9408634025289	11.486876054131\\
2.00122758828403	13.0907373718063\\
-2.00122758828404	13.0907373718063\\
-2.05511900595268	14.6876507099497\\
2.05511900595269	14.6876507099497\\
};
\addlegendentry{right going}

\addplot [color=mycolor2, draw=none, mark=triangle, mark options={solid, mycolor2}]
  table[row sep=crcr]{%
-1.4206909912883	-3.00282300676693\\
1.4206909912883	-3.00282300676693\\
-1.58043854208169	-4.86906922382785\\
1.58043854208169	-4.86906922382785\\
-1.69801972355383	-6.58397118804595\\
1.69801972355383	-6.58397118804595\\
-1.79271597755113	-8.24240167067542\\
1.79271597755113	-8.24240167067542\\
-1.872244836012	-9.8727432041414\\
1.872244836012	-9.8727432041414\\
-1.94086340252889	-11.486876054131\\
1.9408634025289	-11.486876054131\\
-2.00122758828403	-13.0907373718063\\
2.00122758828404	-13.0907373718063\\
2.05511900595268	-14.6876507099497\\
-2.05511900595269	-14.6876507099497\\
};
\addlegendentry{left going}

\addplot [color=black, draw=none, mark=x, mark options={solid, black}]
  table[row sep=crcr]{%
-0.379609792565303	0\\
1.2282514273249	0\\
1.36422627993204	0\\
2.47440307222837	0\\
3.10978768641905	0\\
0.379609792565303	0\\
-1.2282514273249	0\\
-1.36422627993204	0\\
-2.47440307222837	0\\
-3.10978768641905	0\\
};
\addlegendentry{$\Imag(k)=0$}

\end{axis}




\begin{axis}[%
width=3.3in,
height=0.4in,
at={(0in,-1in)},
scale only axis,
xmin=-4,
xlabel={$\Real(k)$},
ylabel={$\omega$}, 
ytick distance=0.05,
grid=major,
xmax=4,
ymin=1.3,
ymax=1.4,
axis background/.style={fill=white},
legend style={at={(3.4in,0.4in)}, anchor=north west, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=black]
  table[row sep=crcr]{%
-0.86	1.326\\
-0.784566539661727	1.32758620689655\\
-0.715269574094674	1.33103448275862\\
-0.667975084090887	1.33448275862069\\
-0.628995965529202	1.33793103448276\\
-0.594736276908402	1.34137931034483\\
-0.563596599650933	1.3448275862069\\
-0.534694761359401	1.34827586206897\\
-0.507478984057304	1.35172413793103\\
-0.481573129809723	1.3551724137931\\
-0.456703400280504	1.35862068965517\\
-0.432659257203021	1.36206896551724\\
-0.409270546630737	1.36551724137931\\
-0.386392923960937	1.36896551724138\\
-0.363897691917939	1.37241379310345\\
-0.341663899575039	1.37586206896552\\
-0.319571303553098	1.37931034482759\\
-0.297493028737222	1.38275862068966\\
-0.275286607895773	1.38620689655172\\
-0.252781414359191	1.38965517241379\\
-0.229758858139499	1.39310344827586\\
-0.205917711018508	1.39655172413793\\
-0.180806227936438	1.4\\
};
\addlegendentry{Rayleigh eq.}

\addplot [color=mycolor1, draw=none, mark=o, mark options={solid, mycolor1}]
  table[row sep=crcr]{%
-0.379609792565303	1.37\\
1.2282514273249	1.37\\
1.36422627993204	1.37\\
2.47440307222837	1.37\\
3.10978768641905	1.37\\
};
\addlegendentry{right going}

\addplot [color=mycolor2, draw=none, mark=triangle, mark options={solid, mycolor2}]
  table[row sep=crcr]{%
0.379609792565303	1.37\\
-1.2282514273249	1.37\\
-1.36422627993204	1.37\\
-2.47440307222837	1.37\\
-3.10978768641905	1.37\\
};
\addlegendentry{left going}

\addplot [color=black]
  table[row sep=crcr]{%
-1.24538497560022	1.3\\
-1.25125349702724	1.30344827586207\\
-1.25711984119107	1.30689655172414\\
-1.26298412602674	1.31034482758621\\
-1.26884646855423	1.31379310344828\\
-1.27470698491847	1.31724137931034\\
-1.2805657904283	1.32068965517241\\
-1.28642299959462	1.32413793103448\\
-1.29227872616762	1.32758620689655\\
-1.29813308317314	1.33103448275862\\
-1.30398618294835	1.33448275862069\\
-1.30983813717655	1.33793103448276\\
-1.31568905692129	1.34137931034483\\
-1.32153905265981	1.3448275862069\\
-1.3273882343157	1.34827586206897\\
-1.33323671129109	1.35172413793103\\
-1.33908459249802	1.3551724137931\\
-1.34493198638938	1.35862068965517\\
-1.35077900098918	1.36206896551724\\
-1.35662574392232	1.36551724137931\\
-1.3624723224438	1.36896551724138\\
-1.36831884346751	1.37241379310345\\
-1.37416541359439	1.37586206896552\\
-1.38001213914031	1.37931034482759\\
-1.38585912616338	1.38275862068966\\
-1.39170648049086	1.38620689655172\\
-1.39755430774572	1.38965517241379\\
-1.40340271337277	1.39310344827586\\
-1.40925180266441	1.39655172413793\\
-1.41510168078606	1.4\\
};

\addplot [color=black]
  table[row sep=crcr]{%
1.24538497560022	1.3\\
1.25125349702724	1.30344827586207\\
1.25711984119107	1.30689655172414\\
1.26298412602674	1.31034482758621\\
1.26884646855423	1.31379310344828\\
1.27470698491847	1.31724137931034\\
1.2805657904283	1.32068965517241\\
1.28642299959462	1.32413793103448\\
1.29227872616762	1.32758620689655\\
1.29813308317314	1.33103448275862\\
1.30398618294835	1.33448275862069\\
1.30983813717655	1.33793103448276\\
1.31568905692129	1.34137931034483\\
1.32153905265981	1.3448275862069\\
1.3273882343157	1.34827586206897\\
1.33323671129109	1.35172413793103\\
1.33908459249802	1.3551724137931\\
1.34493198638938	1.35862068965517\\
1.35077900098918	1.36206896551724\\
1.35662574392232	1.36551724137931\\
1.3624723224438	1.36896551724138\\
1.36831884346751	1.37241379310345\\
1.37416541359439	1.37586206896552\\
1.38001213914031	1.37931034482759\\
1.38585912616338	1.38275862068966\\
1.39170648049086	1.38620689655172\\
1.39755430774572	1.38965517241379\\
1.40340271337277	1.39310344827586\\
1.40925180266441	1.39655172413793\\
1.41510168078606	1.4\\
};

\addplot [color=black]
  table[row sep=crcr]{%
2.96734972376081	1.3\\
2.97435656337979	1.30344827586207\\
2.98136442387078	1.30689655172414\\
2.98837330458452	1.31034482758621\\
2.9953832048533	1.31379310344828\\
3.00239412399132	1.31724137931034\\
3.00940606129505	1.32068965517241\\
3.01641901604358	1.32413793103448\\
3.02343298749898	1.32758620689655\\
3.0304479749066	1.33103448275862\\
3.03746397749545	1.33448275862069\\
3.0444809944785	1.33793103448276\\
3.05149902505301	1.34137931034483\\
3.05851806840084	1.3448275862069\\
3.0655381236888	1.34827586206897\\
3.07255919006888	1.35172413793103\\
3.07958126667864	1.3551724137931\\
3.08660435264145	1.35862068965517\\
3.0936284470668	1.36206896551724\\
3.10065354905058	1.36551724137931\\
3.10767965767538	1.36896551724138\\
3.11470677201074	1.37241379310345\\
3.12173489111345	1.37586206896552\\
3.1287640140278	1.37931034482759\\
3.13579413978586	1.38275862068966\\
3.14282526740772	1.38620689655172\\
3.14985739590176	1.38965517241379\\
3.1568905242649	1.39310344827586\\
3.16392465148284	1.39655172413793\\
3.17095977653031	1.4\\
};

\addplot [color=black]
  table[row sep=crcr]{%
-2.96734972376081	1.3\\
-2.97435656337979	1.30344827586207\\
-2.98136442387078	1.30689655172414\\
-2.98837330458452	1.31034482758621\\
-2.9953832048533	1.31379310344828\\
-3.00239412399132	1.31724137931034\\
-3.00940606129505	1.32068965517241\\
-3.01641901604358	1.32413793103448\\
-3.02343298749898	1.32758620689655\\
-3.0304479749066	1.33103448275862\\
-3.03746397749545	1.33448275862069\\
-3.0444809944785	1.33793103448276\\
-3.05149902505301	1.34137931034483\\
-3.05851806840084	1.3448275862069\\
-3.0655381236888	1.34827586206897\\
-3.07255919006888	1.35172413793103\\
-3.07958126667864	1.3551724137931\\
-3.08660435264145	1.35862068965517\\
-3.0936284470668	1.36206896551724\\
-3.10065354905058	1.36551724137931\\
-3.10767965767538	1.36896551724138\\
-3.11470677201074	1.37241379310345\\
-3.12173489111345	1.37586206896552\\
-3.1287640140278	1.37931034482759\\
-3.13579413978586	1.38275862068966\\
-3.14282526740772	1.38620689655172\\
-3.14985739590176	1.38965517241379\\
-3.1568905242649	1.39310344827586\\
-3.16392465148284	1.39655172413793\\
-3.17095977653031	1.4\\
};

\addplot [color=black]
  table[row sep=crcr]{%
2.23331129543969	1.3\\
2.2456099189327	1.30344827586207\\
2.25786587195479	1.30689655172414\\
2.27007867670025	1.31034482758621\\
2.28224794427973	1.31379310344828\\
2.2943733678611	1.31724137931034\\
2.3064547161917	1.32068965517241\\
2.31849182749742	1.32413793103448\\
2.33048460375079	1.32758620689655\\
2.34243300529783	1.33103448275862\\
2.35433704583153	1.33448275862069\\
2.36619678769857	1.33793103448276\\
2.37801233752467	1.34137931034483\\
2.38978384214373	1.3448275862069\\
2.40151148481505	1.34827586206897\\
2.41319548171356	1.35172413793103\\
2.42483607867721	1.3551724137931\\
2.43643354819682	1.35862068965517\\
2.44798818663329	1.36206896551724\\
2.45950031164808	1.36551724137931\\
2.47097025983314	1.36896551724138\\
2.48239838452703	1.37241379310345\\
2.49378505380475	1.37586206896552\\
2.50513064862927	1.37931034482759\\
2.51643556115347	1.38275862068966\\
2.52770019316178	1.38620689655172\\
2.53892495464151	1.38965517241379\\
2.55011026247428	1.39310344827586\\
2.56125653923894	1.39655172413793\\
2.57236421211736	1.4\\
};

\addplot [color=black]
  table[row sep=crcr]{%
-2.23331129543969	1.3\\
-2.2456099189327	1.30344827586207\\
-2.25786587195479	1.30689655172414\\
-2.27007867670025	1.31034482758621\\
-2.28224794427973	1.31379310344828\\
-2.2943733678611	1.31724137931034\\
-2.3064547161917	1.32068965517241\\
-2.31849182749742	1.32413793103448\\
-2.33048460375079	1.32758620689655\\
-2.34243300529783	1.33103448275862\\
-2.35433704583153	1.33448275862069\\
-2.36619678769857	1.33793103448276\\
-2.37801233752467	1.34137931034483\\
-2.38978384214373	1.3448275862069\\
-2.40151148481505	1.34827586206897\\
-2.41319548171356	1.35172413793103\\
-2.42483607867721	1.3551724137931\\
-2.43643354819682	1.35862068965517\\
-2.44798818663329	1.36206896551724\\
-2.45950031164808	1.36551724137931\\
-2.47097025983314	1.36896551724138\\
-2.48239838452703	1.37241379310345\\
-2.49378505380475	1.37586206896552\\
-2.50513064862927	1.37931034482759\\
-2.51643556115347	1.38275862068966\\
-2.52770019316178	1.38620689655172\\
-2.53892495464151	1.38965517241379\\
-2.55011026247428	1.39310344827586\\
-2.56125653923894	1.39655172413793\\
-2.57236421211736	1.4\\
};

\addplot [color=black]
  table[row sep=crcr]{%
0.86	1.326\\
0.929412739415687	1.32758620689655\\
0.990545483281801	1.33103448275862\\
1.02963393518102	1.33448275862069\\
1.06035711042955	1.33793103448276\\
1.08630175112185	1.34137931034483\\
1.10905677557982	1.3448275862069\\
1.12949231819793	1.34827586206897\\
1.14814628364591	1.35172413793103\\
1.16537872377472	1.3551724137931\\
1.18144465376449	1.35862068965517\\
1.19653250228011	1.36206896551724\\
1.21078615728211	1.36551724137931\\
1.22431842821669	1.36896551724138\\
1.23721968726884	1.37241379310345\\
1.24956364576018	1.37586206896552\\
1.26141134771563	1.37931034482759\\
1.27281401043963	1.38275862068966\\
1.28381509472055	1.38620689655172\\
1.29445184569351	1.38965517241379\\
1.30475646102415	1.39310344827586\\
1.31475699105245	1.39655172413793\\
1.32447804248352	1.4\\
};

\addplot [color=black]
  table[row sep=crcr]{%
0.86	1.326\\
0.784566539661727	1.32758620689655\\
0.715269574094674	1.33103448275862\\
0.667975084090887	1.33448275862069\\
0.628995965529202	1.33793103448276\\
0.594736276908402	1.34137931034483\\
0.563596599650933	1.3448275862069\\
0.534694761359401	1.34827586206897\\
0.507478984057304	1.35172413793103\\
0.481573129809723	1.3551724137931\\
0.456703400280504	1.35862068965517\\
0.432659257203021	1.36206896551724\\
0.409270546630737	1.36551724137931\\
0.386392923960937	1.36896551724138\\
0.363897691917939	1.37241379310345\\
0.341663899575039	1.37586206896552\\
0.319571303553098	1.37931034482759\\
0.297493028737222	1.38275862068966\\
0.275286607895773	1.38620689655172\\
0.252781414359191	1.38965517241379\\
0.229758858139499	1.39310344827586\\
0.205917711018508	1.39655172413793\\
0.180806227936438	1.4\\
};

\addplot [color=black]
  table[row sep=crcr]{%
-0.86	1.326\\
-0.929412739415687	1.32758620689655\\
-0.990545483281801	1.33103448275862\\
-1.02963393518102	1.33448275862069\\
-1.06035711042955	1.33793103448276\\
-1.08630175112185	1.34137931034483\\
-1.10905677557982	1.3448275862069\\
-1.12949231819793	1.34827586206897\\
-1.14814628364591	1.35172413793103\\
-1.16537872377472	1.3551724137931\\
-1.18144465376449	1.35862068965517\\
-1.19653250228011	1.36206896551724\\
-1.21078615728211	1.36551724137931\\
-1.22431842821669	1.36896551724138\\
-1.23721968726884	1.37241379310345\\
-1.24956364576018	1.37586206896552\\
-1.26141134771563	1.37931034482759\\
-1.27281401043963	1.38275862068966\\
-1.28381509472055	1.38620689655172\\
-1.29445184569351	1.38965517241379\\
-1.30475646102415	1.39310344827586\\
-1.31475699105245	1.39655172413793\\
-1.32447804248352	1.4\\
};

\end{axis}
\end{tikzpicture}%

==> [4] Elastic problem in regular waveguides/rcmode2.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.49400,0.18400,0.55600}%
\definecolor{mycolor2}{rgb}{0.46600,0.67400,0.18800}%
%
\begin{tikzpicture}

\begin{axis}[%
width=6.297in,
height=0.933in,
at={(1.056in,0.236in)},
scale only axis,
xmin=-4,
xmax=4,
ymin=1.3,
ymax=1.4,
axis background/.style={fill=white},
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=black]
  table[row sep=crcr]{%
-0.86	1.326\\
-0.784566539661727	1.32758620689655\\
-0.715269574094674	1.33103448275862\\
-0.667975084090887	1.33448275862069\\
-0.628995965529202	1.33793103448276\\
-0.594736276908402	1.34137931034483\\
-0.563596599650933	1.3448275862069\\
-0.534694761359401	1.34827586206897\\
-0.507478984057304	1.35172413793103\\
-0.481573129809723	1.3551724137931\\
-0.456703400280504	1.35862068965517\\
-0.432659257203021	1.36206896551724\\
-0.409270546630737	1.36551724137931\\
-0.386392923960937	1.36896551724138\\
-0.363897691917939	1.37241379310345\\
-0.341663899575039	1.37586206896552\\
-0.319571303553098	1.37931034482759\\
-0.297493028737222	1.38275862068966\\
-0.275286607895773	1.38620689655172\\
-0.252781414359191	1.38965517241379\\
-0.229758858139499	1.39310344827586\\
-0.205917711018508	1.39655172413793\\
-0.180806227936438	1.4\\
};
\addlegendentry{data1}

\addplot [color=black]
  table[row sep=crcr]{%
-1.24538497560022	1.3\\
-1.25125349702724	1.30344827586207\\
-1.25711984119107	1.30689655172414\\
-1.26298412602674	1.31034482758621\\
-1.26884646855423	1.31379310344828\\
-1.27470698491847	1.31724137931034\\
-1.2805657904283	1.32068965517241\\
-1.28642299959462	1.32413793103448\\
-1.29227872616762	1.32758620689655\\
-1.29813308317314	1.33103448275862\\
-1.30398618294835	1.33448275862069\\
-1.30983813717655	1.33793103448276\\
-1.31568905692129	1.34137931034483\\
-1.32153905265981	1.3448275862069\\
-1.3273882343157	1.34827586206897\\
-1.33323671129109	1.35172413793103\\
-1.33908459249802	1.3551724137931\\
-1.34493198638938	1.35862068965517\\
-1.35077900098918	1.36206896551724\\
-1.35662574392232	1.36551724137931\\
-1.3624723224438	1.36896551724138\\
-1.36831884346751	1.37241379310345\\
-1.37416541359439	1.37586206896552\\
-1.38001213914031	1.37931034482759\\
-1.38585912616338	1.38275862068966\\
-1.39170648049086	1.38620689655172\\
-1.39755430774572	1.38965517241379\\
-1.40340271337277	1.39310344827586\\
-1.40925180266441	1.39655172413793\\
-1.41510168078606	1.4\\
};
\addlegendentry{data2}

\addplot [color=black]
  table[row sep=crcr]{%
1.24538497560022	1.3\\
1.25125349702724	1.30344827586207\\
1.25711984119107	1.30689655172414\\
1.26298412602674	1.31034482758621\\
1.26884646855423	1.31379310344828\\
1.27470698491847	1.31724137931034\\
1.2805657904283	1.32068965517241\\
1.28642299959462	1.32413793103448\\
1.29227872616762	1.32758620689655\\
1.29813308317314	1.33103448275862\\
1.30398618294835	1.33448275862069\\
1.30983813717655	1.33793103448276\\
1.31568905692129	1.34137931034483\\
1.32153905265981	1.3448275862069\\
1.3273882343157	1.34827586206897\\
1.33323671129109	1.35172413793103\\
1.33908459249802	1.3551724137931\\
1.34493198638938	1.35862068965517\\
1.35077900098918	1.36206896551724\\
1.35662574392232	1.36551724137931\\
1.3624723224438	1.36896551724138\\
1.36831884346751	1.37241379310345\\
1.37416541359439	1.37586206896552\\
1.38001213914031	1.37931034482759\\
1.38585912616338	1.38275862068966\\
1.39170648049086	1.38620689655172\\
1.39755430774572	1.38965517241379\\
1.40340271337277	1.39310344827586\\
1.40925180266441	1.39655172413793\\
1.41510168078606	1.4\\
};
\addlegendentry{data3}

\addplot [color=black]
  table[row sep=crcr]{%
2.96734972376081	1.3\\
2.97435656337979	1.30344827586207\\
2.98136442387078	1.30689655172414\\
2.98837330458452	1.31034482758621\\
2.9953832048533	1.31379310344828\\
3.00239412399132	1.31724137931034\\
3.00940606129505	1.32068965517241\\
3.01641901604358	1.32413793103448\\
3.02343298749898	1.32758620689655\\
3.0304479749066	1.33103448275862\\
3.03746397749545	1.33448275862069\\
3.0444809944785	1.33793103448276\\
3.05149902505301	1.34137931034483\\
3.05851806840084	1.3448275862069\\
3.0655381236888	1.34827586206897\\
3.07255919006888	1.35172413793103\\
3.07958126667864	1.3551724137931\\
3.08660435264145	1.35862068965517\\
3.0936284470668	1.36206896551724\\
3.10065354905058	1.36551724137931\\
3.10767965767538	1.36896551724138\\
3.11470677201074	1.37241379310345\\
3.12173489111345	1.37586206896552\\
3.1287640140278	1.37931034482759\\
3.13579413978586	1.38275862068966\\
3.14282526740772	1.38620689655172\\
3.14985739590176	1.38965517241379\\
3.1568905242649	1.39310344827586\\
3.16392465148284	1.39655172413793\\
3.17095977653031	1.4\\
};
\addlegendentry{data4}

\addplot [color=black]
  table[row sep=crcr]{%
-2.96734972376081	1.3\\
-2.97435656337979	1.30344827586207\\
-2.98136442387078	1.30689655172414\\
-2.98837330458452	1.31034482758621\\
-2.9953832048533	1.31379310344828\\
-3.00239412399132	1.31724137931034\\
-3.00940606129505	1.32068965517241\\
-3.01641901604358	1.32413793103448\\
-3.02343298749898	1.32758620689655\\
-3.0304479749066	1.33103448275862\\
-3.03746397749545	1.33448275862069\\
-3.0444809944785	1.33793103448276\\
-3.05149902505301	1.34137931034483\\
-3.05851806840084	1.3448275862069\\
-3.0655381236888	1.34827586206897\\
-3.07255919006888	1.35172413793103\\
-3.07958126667864	1.3551724137931\\
-3.08660435264145	1.35862068965517\\
-3.0936284470668	1.36206896551724\\
-3.10065354905058	1.36551724137931\\
-3.10767965767538	1.36896551724138\\
-3.11470677201074	1.37241379310345\\
-3.12173489111345	1.37586206896552\\
-3.1287640140278	1.37931034482759\\
-3.13579413978586	1.38275862068966\\
-3.14282526740772	1.38620689655172\\
-3.14985739590176	1.38965517241379\\
-3.1568905242649	1.39310344827586\\
-3.16392465148284	1.39655172413793\\
-3.17095977653031	1.4\\
};
\addlegendentry{data5}

\addplot [color=black]
  table[row sep=crcr]{%
2.23331129543969	1.3\\
2.2456099189327	1.30344827586207\\
2.25786587195479	1.30689655172414\\
2.27007867670025	1.31034482758621\\
2.28224794427973	1.31379310344828\\
2.2943733678611	1.31724137931034\\
2.3064547161917	1.32068965517241\\
2.31849182749742	1.32413793103448\\
2.33048460375079	1.32758620689655\\
2.34243300529783	1.33103448275862\\
2.35433704583153	1.33448275862069\\
2.36619678769857	1.33793103448276\\
2.37801233752467	1.34137931034483\\
2.38978384214373	1.3448275862069\\
2.40151148481505	1.34827586206897\\
2.41319548171356	1.35172413793103\\
2.42483607867721	1.3551724137931\\
2.43643354819682	1.35862068965517\\
2.44798818663329	1.36206896551724\\
2.45950031164808	1.36551724137931\\
2.47097025983314	1.36896551724138\\
2.48239838452703	1.37241379310345\\
2.49378505380475	1.37586206896552\\
2.50513064862927	1.37931034482759\\
2.51643556115347	1.38275862068966\\
2.52770019316178	1.38620689655172\\
2.53892495464151	1.38965517241379\\
2.55011026247428	1.39310344827586\\
2.56125653923894	1.39655172413793\\
2.57236421211736	1.4\\
};
\addlegendentry{data6}

\addplot [color=black]
  table[row sep=crcr]{%
-2.23331129543969	1.3\\
-2.2456099189327	1.30344827586207\\
-2.25786587195479	1.30689655172414\\
-2.27007867670025	1.31034482758621\\
-2.28224794427973	1.31379310344828\\
-2.2943733678611	1.31724137931034\\
-2.3064547161917	1.32068965517241\\
-2.31849182749742	1.32413793103448\\
-2.33048460375079	1.32758620689655\\
-2.34243300529783	1.33103448275862\\
-2.35433704583153	1.33448275862069\\
-2.36619678769857	1.33793103448276\\
-2.37801233752467	1.34137931034483\\
-2.38978384214373	1.3448275862069\\
-2.40151148481505	1.34827586206897\\
-2.41319548171356	1.35172413793103\\
-2.42483607867721	1.3551724137931\\
-2.43643354819682	1.35862068965517\\
-2.44798818663329	1.36206896551724\\
-2.45950031164808	1.36551724137931\\
-2.47097025983314	1.36896551724138\\
-2.48239838452703	1.37241379310345\\
-2.49378505380475	1.37586206896552\\
-2.50513064862927	1.37931034482759\\
-2.51643556115347	1.38275862068966\\
-2.52770019316178	1.38620689655172\\
-2.53892495464151	1.38965517241379\\
-2.55011026247428	1.39310344827586\\
-2.56125653923894	1.39655172413793\\
-2.57236421211736	1.4\\
};
\addlegendentry{data7}

\addplot [color=black]
  table[row sep=crcr]{%
0.86	1.326\\
0.929412739415687	1.32758620689655\\
0.990545483281801	1.33103448275862\\
1.02963393518102	1.33448275862069\\
1.06035711042955	1.33793103448276\\
1.08630175112185	1.34137931034483\\
1.10905677557982	1.3448275862069\\
1.12949231819793	1.34827586206897\\
1.14814628364591	1.35172413793103\\
1.16537872377472	1.3551724137931\\
1.18144465376449	1.35862068965517\\
1.19653250228011	1.36206896551724\\
1.21078615728211	1.36551724137931\\
1.22431842821669	1.36896551724138\\
1.23721968726884	1.37241379310345\\
1.24956364576018	1.37586206896552\\
1.26141134771563	1.37931034482759\\
1.27281401043963	1.38275862068966\\
1.28381509472055	1.38620689655172\\
1.29445184569351	1.38965517241379\\
1.30475646102415	1.39310344827586\\
1.31475699105245	1.39655172413793\\
1.32447804248352	1.4\\
};
\addlegendentry{data8}

\addplot [color=black]
  table[row sep=crcr]{%
0.86	1.326\\
0.784566539661727	1.32758620689655\\
0.715269574094674	1.33103448275862\\
0.667975084090887	1.33448275862069\\
0.628995965529202	1.33793103448276\\
0.594736276908402	1.34137931034483\\
0.563596599650933	1.3448275862069\\
0.534694761359401	1.34827586206897\\
0.507478984057304	1.35172413793103\\
0.481573129809723	1.3551724137931\\
0.456703400280504	1.35862068965517\\
0.432659257203021	1.36206896551724\\
0.409270546630737	1.36551724137931\\
0.386392923960937	1.36896551724138\\
0.363897691917939	1.37241379310345\\
0.341663899575039	1.37586206896552\\
0.319571303553098	1.37931034482759\\
0.297493028737222	1.38275862068966\\
0.275286607895773	1.38620689655172\\
0.252781414359191	1.38965517241379\\
0.229758858139499	1.39310344827586\\
0.205917711018508	1.39655172413793\\
0.180806227936438	1.4\\
};
\addlegendentry{data9}

\addplot [color=black]
  table[row sep=crcr]{%
-0.86	1.326\\
-0.929412739415687	1.32758620689655\\
-0.990545483281801	1.33103448275862\\
-1.02963393518102	1.33448275862069\\
-1.06035711042955	1.33793103448276\\
-1.08630175112185	1.34137931034483\\
-1.10905677557982	1.3448275862069\\
-1.12949231819793	1.34827586206897\\
-1.14814628364591	1.35172413793103\\
-1.16537872377472	1.3551724137931\\
-1.18144465376449	1.35862068965517\\
-1.19653250228011	1.36206896551724\\
-1.21078615728211	1.36551724137931\\
-1.22431842821669	1.36896551724138\\
-1.23721968726884	1.37241379310345\\
-1.24956364576018	1.37586206896552\\
-1.26141134771563	1.37931034482759\\
-1.27281401043963	1.38275862068966\\
-1.28381509472055	1.38620689655172\\
-1.29445184569351	1.38965517241379\\
-1.30475646102415	1.39310344827586\\
-1.31475699105245	1.39655172413793\\
-1.32447804248352	1.4\\
};
\addlegendentry{data10}

\addplot [color=mycolor1, draw=none, mark=o, mark options={solid, mycolor1}]
  table[row sep=crcr]{%
-0.379609792565303	1.37\\
1.2282514273249	1.37\\
1.36422627993204	1.37\\
2.47440307222837	1.37\\
3.10978768641905	1.37\\
};
\addlegendentry{data11}

\addplot [color=mycolor2, draw=none, mark=triangle, mark options={solid, mycolor2}]
  table[row sep=crcr]{%
0.379609792565303	1.37\\
-1.2282514273249	1.37\\
-1.36422627993204	1.37\\
-2.47440307222837	1.37\\
-3.10978768641905	1.37\\
};
\addlegendentry{data12}

\end{axis}
\end{tikzpicture}%

==> [4] Elastic problem in regular waveguides/source2D.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\addplot [color=red,style={ultra thick}]
  table[row sep=crcr]{%
-0.5	0.06\\
-0.47979797979798	0.0570001530495116\\
-0.45959595959596	0.0557792762796412\\
-0.439393939393939	0.0548574052277342\\
-0.419191919191919	0.054092851912237\\
-0.398989898989899	0.0534304595791882\\
-0.378787878787879	0.0528418110236256\\
-0.358585858585859	0.0523099530057882\\
-0.338383838383838	0.051823795416223\\
-0.318181818181818	0.051375606381359\\
-0.297979797979798	0.0509597370362568\\
-0.277777777777778	0.0505719095841794\\
-0.257575757575758	0.0502087912597554\\
-0.237373737373737	0.0498677251531512\\
-0.217171717171717	0.0495465525389937\\
-0.196969696969697	0.0492434913034552\\
-0.176767676767677	0.0489570502070978\\
-0.156565656565657	0.0486859668469124\\
-0.136363636363636	0.0484291617624019\\
-0.116161616161616	0.048185703824474\\
-0.095959595959596	0.0479547836882716\\
-0.0757575757575757	0.0477356931243345\\
-0.0555555555555556	0.0475278087107535\\
-0.0353535353535354	0.0473305788118989\\
-0.0151515151515151	0.0471435130693355\\
0.00505050505050508	0.0469661738378142\\
0.0252525252525253	0.0467981691449746\\
0.0454545454545454	0.0466391468575463\\
0.0656565656565656	0.0464887898123588\\
0.0858585858585859	0.0463468117259772\\
0.106060606060606	0.0462129537380881\\
0.126262626262626	0.0460869814748497\\
0.146464646464647	0.0459686825420725\\
0.166666666666667	0.045857864376269\\
0.186868686868687	0.0457543523957053\\
0.207070707070707	0.045657988404607\\
0.227272727272727	0.045568629212375\\
0.247474747474748	0.0454861454365721\\
0.267676767676768	0.045410420463987\\
0.287878787878788	0.0453413495485481\\
0.308080808080808	0.0452788390284956\\
0.328282828282828	0.045222805648198\\
0.348484848484849	0.0451731759724545\\
0.368686868686869	0.0451298858831693\\
0.388888888888889	0.0450928801500014\\
0.409090909090909	0.0450621120680409\\
0.429292929292929	0.0450375431568139\\
0.44949494949495	0.04501914291599\\
0.46969696969697	0.0450068886341176\\
0.48989898989899	0.0450007652475581\\
0.51010101010101	0.0450007652475581\\
0.53030303030303	0.0450068886341176\\
0.550505050505051	0.04501914291599\\
0.570707070707071	0.0450375431568139\\
0.590909090909091	0.0450621120680409\\
0.611111111111111	0.0450928801500014\\
0.631313131313131	0.0451298858831693\\
0.651515151515152	0.0451731759724545\\
0.671717171717172	0.045222805648198\\
0.691919191919192	0.0452788390284956\\
0.712121212121212	0.0453413495485481\\
0.732323232323232	0.045410420463987\\
0.752525252525253	0.0454861454365721\\
0.772727272727273	0.045568629212375\\
0.792929292929293	0.045657988404607\\
0.813131313131313	0.0457543523957053\\
0.833333333333333	0.045857864376269\\
0.853535353535354	0.0459686825420725\\
0.873737373737374	0.0460869814748497\\
0.893939393939394	0.0462129537380881\\
0.914141414141414	0.0463468117259772\\
0.934343434343434	0.0464887898123588\\
0.954545454545455	0.0466391468575463\\
0.974747474747475	0.0467981691449746\\
0.994949494949495	0.0469661738378142\\
1.01515151515152	0.0471435130693355\\
1.03535353535354	0.0473305788118989\\
1.05555555555556	0.0475278087107535\\
1.07575757575758	0.0477356931243345\\
1.0959595959596	0.0479547836882716\\
1.11616161616162	0.048185703824474\\
1.13636363636364	0.048429161762402\\
1.15656565656566	0.0486859668469124\\
1.17676767676768	0.0489570502070978\\
1.1969696969697	0.0492434913034552\\
1.21717171717172	0.0495465525389937\\
1.23737373737374	0.0498677251531512\\
1.25757575757576	0.0502087912597554\\
1.27777777777778	0.0505719095841794\\
1.2979797979798	0.0509597370362568\\
1.31818181818182	0.051375606381359\\
1.33838383838384	0.051823795416223\\
1.35858585858586	0.0523099530057882\\
1.37878787878788	0.0528418110236256\\
1.3989898989899	0.0534304595791882\\
1.41919191919192	0.054092851912237\\
1.43939393939394	0.0548574052277342\\
1.45959595959596	0.0557792762796412\\
1.47979797979798	0.0570001530495116\\
1.5	0.06\\
};

\addplot [color=red,style={ultra thick}]
  table[row sep=crcr]{%
-0.5	0.06\\
-0.47979797979798	0.0629998469504884\\
-0.45959595959596	0.0642207237203588\\
-0.439393939393939	0.0651425947722658\\
-0.419191919191919	0.065907148087763\\
-0.398989898989899	0.0665695404208118\\
-0.378787878787879	0.0671581889763744\\
-0.358585858585859	0.0676900469942118\\
-0.338383838383838	0.068176204583777\\
-0.318181818181818	0.068624393618641\\
-0.297979797979798	0.0690402629637432\\
-0.277777777777778	0.0694280904158206\\
-0.257575757575758	0.0697912087402446\\
-0.237373737373737	0.0701322748468488\\
-0.217171717171717	0.0704534474610063\\
-0.196969696969697	0.0707565086965447\\
-0.176767676767677	0.0710429497929022\\
-0.156565656565657	0.0713140331530876\\
-0.136363636363636	0.0715708382375981\\
-0.116161616161616	0.071814296175526\\
-0.095959595959596	0.0720452163117284\\
-0.0757575757575757	0.0722643068756655\\
-0.0555555555555556	0.0724721912892465\\
-0.0353535353535354	0.0726694211881011\\
-0.0151515151515151	0.0728564869306645\\
0.00505050505050508	0.0730338261621858\\
0.0252525252525253	0.0732018308550254\\
0.0454545454545454	0.0733608531424537\\
0.0656565656565656	0.0735112101876412\\
0.0858585858585859	0.0736531882740228\\
0.106060606060606	0.0737870462619119\\
0.126262626262626	0.0739130185251503\\
0.146464646464647	0.0740313174579275\\
0.166666666666667	0.074142135623731\\
0.186868686868687	0.0742456476042947\\
0.207070707070707	0.074342011595393\\
0.227272727272727	0.074431370787625\\
0.247474747474748	0.0745138545634279\\
0.267676767676768	0.074589579536013\\
0.287878787878788	0.0746586504514519\\
0.308080808080808	0.0747211609715044\\
0.328282828282828	0.0747771943518019\\
0.348484848484849	0.0748268240275455\\
0.368686868686869	0.0748701141168307\\
0.388888888888889	0.0749071198499986\\
0.409090909090909	0.0749378879319591\\
0.429292929292929	0.0749624568431861\\
0.44949494949495	0.07498085708401\\
0.46969696969697	0.0749931113658824\\
0.48989898989899	0.0749992347524419\\
0.51010101010101	0.0749992347524419\\
0.53030303030303	0.0749931113658824\\
0.550505050505051	0.07498085708401\\
0.570707070707071	0.0749624568431861\\
0.590909090909091	0.0749378879319591\\
0.611111111111111	0.0749071198499986\\
0.631313131313131	0.0748701141168307\\
0.651515151515152	0.0748268240275455\\
0.671717171717172	0.0747771943518019\\
0.691919191919192	0.0747211609715044\\
0.712121212121212	0.0746586504514519\\
0.732323232323232	0.074589579536013\\
0.752525252525253	0.0745138545634279\\
0.772727272727273	0.074431370787625\\
0.792929292929293	0.074342011595393\\
0.813131313131313	0.0742456476042947\\
0.833333333333333	0.074142135623731\\
0.853535353535354	0.0740313174579275\\
0.873737373737374	0.0739130185251503\\
0.893939393939394	0.0737870462619119\\
0.914141414141414	0.0736531882740228\\
0.934343434343434	0.0735112101876412\\
0.954545454545455	0.0733608531424537\\
0.974747474747475	0.0732018308550254\\
0.994949494949495	0.0730338261621858\\
1.01515151515152	0.0728564869306645\\
1.03535353535354	0.0726694211881011\\
1.05555555555556	0.0724721912892465\\
1.07575757575758	0.0722643068756655\\
1.0959595959596	0.0720452163117284\\
1.11616161616162	0.071814296175526\\
1.13636363636364	0.0715708382375981\\
1.15656565656566	0.0713140331530876\\
1.17676767676768	0.0710429497929022\\
1.1969696969697	0.0707565086965447\\
1.21717171717172	0.0704534474610063\\
1.23737373737374	0.0701322748468488\\
1.25757575757576	0.0697912087402446\\
1.27777777777778	0.0694280904158206\\
1.2979797979798	0.0690402629637432\\
1.31818181818182	0.068624393618641\\
1.33838383838384	0.068176204583777\\
1.35858585858586	0.0676900469942118\\
1.37878787878788	0.0671581889763744\\
1.3989898989899	0.0665695404208118\\
1.41919191919192	0.065907148087763\\
1.43939393939394	0.0651425947722658\\
1.45959595959596	0.0642207237203588\\
1.47979797979798	0.0629998469504884\\
1.5	0.06\\
};


\addplot [color=red,style={ultra thick}]
  table[row sep=crcr]{%
0.23	0.1\\
0.29	0.1\\
0.35	0.1\\
0.41	0.1\\
0.47	0.1\\
0.53	0.1\\
0.59	0.1\\
0.65	0.1\\
0.71	0.1\\
0.77	0.1\\
};


\addplot [color=red,style={ultra thick}]
  table[row sep=crcr]{%
2	-0.1\\
2.05555555555556	-0.1\\
2.11111111111111	-0.1\\
2.16666666666667	-0.1\\
2.22222222222222	-0.1\\
2.27777777777778	-0.1\\
2.33333333333333	-0.1\\
2.38888888888889	-0.1\\
2.44444444444444	-0.1\\
2.5	-0.1\\
};


==> rcmode2.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.49400,0.18400,0.55600}%
\definecolor{mycolor2}{rgb}{0.46600,0.67400,0.18800}%
%
\begin{tikzpicture}

\begin{axis}[%
width=6.297in,
height=0.933in,
at={(1.056in,0.236in)},
scale only axis,
xmin=-4,
xmax=4,
ymin=1.3,
ymax=1.4,
axis background/.style={fill=white},
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=black]
  table[row sep=crcr]{%
-0.86	1.326\\
-0.784566539661727	1.32758620689655\\
-0.715269574094674	1.33103448275862\\
-0.667975084090887	1.33448275862069\\
-0.628995965529202	1.33793103448276\\
-0.594736276908402	1.34137931034483\\
-0.563596599650933	1.3448275862069\\
-0.534694761359401	1.34827586206897\\
-0.507478984057304	1.35172413793103\\
-0.481573129809723	1.3551724137931\\
-0.456703400280504	1.35862068965517\\
-0.432659257203021	1.36206896551724\\
-0.409270546630737	1.36551724137931\\
-0.386392923960937	1.36896551724138\\
-0.363897691917939	1.37241379310345\\
-0.341663899575039	1.37586206896552\\
-0.319571303553098	1.37931034482759\\
-0.297493028737222	1.38275862068966\\
-0.275286607895773	1.38620689655172\\
-0.252781414359191	1.38965517241379\\
-0.229758858139499	1.39310344827586\\
-0.205917711018508	1.39655172413793\\
-0.180806227936438	1.4\\
};
\addlegendentry{data1}

\addplot [color=black]
  table[row sep=crcr]{%
-1.24538497560022	1.3\\
-1.25125349702724	1.30344827586207\\
-1.25711984119107	1.30689655172414\\
-1.26298412602674	1.31034482758621\\
-1.26884646855423	1.31379310344828\\
-1.27470698491847	1.31724137931034\\
-1.2805657904283	1.32068965517241\\
-1.28642299959462	1.32413793103448\\
-1.29227872616762	1.32758620689655\\
-1.29813308317314	1.33103448275862\\
-1.30398618294835	1.33448275862069\\
-1.30983813717655	1.33793103448276\\
-1.31568905692129	1.34137931034483\\
-1.32153905265981	1.3448275862069\\
-1.3273882343157	1.34827586206897\\
-1.33323671129109	1.35172413793103\\
-1.33908459249802	1.3551724137931\\
-1.34493198638938	1.35862068965517\\
-1.35077900098918	1.36206896551724\\
-1.35662574392232	1.36551724137931\\
-1.3624723224438	1.36896551724138\\
-1.36831884346751	1.37241379310345\\
-1.37416541359439	1.37586206896552\\
-1.38001213914031	1.37931034482759\\
-1.38585912616338	1.38275862068966\\
-1.39170648049086	1.38620689655172\\
-1.39755430774572	1.38965517241379\\
-1.40340271337277	1.39310344827586\\
-1.40925180266441	1.39655172413793\\
-1.41510168078606	1.4\\
};
\addlegendentry{data2}

\addplot [color=black]
  table[row sep=crcr]{%
1.24538497560022	1.3\\
1.25125349702724	1.30344827586207\\
1.25711984119107	1.30689655172414\\
1.26298412602674	1.31034482758621\\
1.26884646855423	1.31379310344828\\
1.27470698491847	1.31724137931034\\
1.2805657904283	1.32068965517241\\
1.28642299959462	1.32413793103448\\
1.29227872616762	1.32758620689655\\
1.29813308317314	1.33103448275862\\
1.30398618294835	1.33448275862069\\
1.30983813717655	1.33793103448276\\
1.31568905692129	1.34137931034483\\
1.32153905265981	1.3448275862069\\
1.3273882343157	1.34827586206897\\
1.33323671129109	1.35172413793103\\
1.33908459249802	1.3551724137931\\
1.34493198638938	1.35862068965517\\
1.35077900098918	1.36206896551724\\
1.35662574392232	1.36551724137931\\
1.3624723224438	1.36896551724138\\
1.36831884346751	1.37241379310345\\
1.37416541359439	1.37586206896552\\
1.38001213914031	1.37931034482759\\
1.38585912616338	1.38275862068966\\
1.39170648049086	1.38620689655172\\
1.39755430774572	1.38965517241379\\
1.40340271337277	1.39310344827586\\
1.40925180266441	1.39655172413793\\
1.41510168078606	1.4\\
};
\addlegendentry{data3}

\addplot [color=black]
  table[row sep=crcr]{%
2.96734972376081	1.3\\
2.97435656337979	1.30344827586207\\
2.98136442387078	1.30689655172414\\
2.98837330458452	1.31034482758621\\
2.9953832048533	1.31379310344828\\
3.00239412399132	1.31724137931034\\
3.00940606129505	1.32068965517241\\
3.01641901604358	1.32413793103448\\
3.02343298749898	1.32758620689655\\
3.0304479749066	1.33103448275862\\
3.03746397749545	1.33448275862069\\
3.0444809944785	1.33793103448276\\
3.05149902505301	1.34137931034483\\
3.05851806840084	1.3448275862069\\
3.0655381236888	1.34827586206897\\
3.07255919006888	1.35172413793103\\
3.07958126667864	1.3551724137931\\
3.08660435264145	1.35862068965517\\
3.0936284470668	1.36206896551724\\
3.10065354905058	1.36551724137931\\
3.10767965767538	1.36896551724138\\
3.11470677201074	1.37241379310345\\
3.12173489111345	1.37586206896552\\
3.1287640140278	1.37931034482759\\
3.13579413978586	1.38275862068966\\
3.14282526740772	1.38620689655172\\
3.14985739590176	1.38965517241379\\
3.1568905242649	1.39310344827586\\
3.16392465148284	1.39655172413793\\
3.17095977653031	1.4\\
};
\addlegendentry{data4}

\addplot [color=black]
  table[row sep=crcr]{%
-2.96734972376081	1.3\\
-2.97435656337979	1.30344827586207\\
-2.98136442387078	1.30689655172414\\
-2.98837330458452	1.31034482758621\\
-2.9953832048533	1.31379310344828\\
-3.00239412399132	1.31724137931034\\
-3.00940606129505	1.32068965517241\\
-3.01641901604358	1.32413793103448\\
-3.02343298749898	1.32758620689655\\
-3.0304479749066	1.33103448275862\\
-3.03746397749545	1.33448275862069\\
-3.0444809944785	1.33793103448276\\
-3.05149902505301	1.34137931034483\\
-3.05851806840084	1.3448275862069\\
-3.0655381236888	1.34827586206897\\
-3.07255919006888	1.35172413793103\\
-3.07958126667864	1.3551724137931\\
-3.08660435264145	1.35862068965517\\
-3.0936284470668	1.36206896551724\\
-3.10065354905058	1.36551724137931\\
-3.10767965767538	1.36896551724138\\
-3.11470677201074	1.37241379310345\\
-3.12173489111345	1.37586206896552\\
-3.1287640140278	1.37931034482759\\
-3.13579413978586	1.38275862068966\\
-3.14282526740772	1.38620689655172\\
-3.14985739590176	1.38965517241379\\
-3.1568905242649	1.39310344827586\\
-3.16392465148284	1.39655172413793\\
-3.17095977653031	1.4\\
};
\addlegendentry{data5}

\addplot [color=black]
  table[row sep=crcr]{%
2.23331129543969	1.3\\
2.2456099189327	1.30344827586207\\
2.25786587195479	1.30689655172414\\
2.27007867670025	1.31034482758621\\
2.28224794427973	1.31379310344828\\
2.2943733678611	1.31724137931034\\
2.3064547161917	1.32068965517241\\
2.31849182749742	1.32413793103448\\
2.33048460375079	1.32758620689655\\
2.34243300529783	1.33103448275862\\
2.35433704583153	1.33448275862069\\
2.36619678769857	1.33793103448276\\
2.37801233752467	1.34137931034483\\
2.38978384214373	1.3448275862069\\
2.40151148481505	1.34827586206897\\
2.41319548171356	1.35172413793103\\
2.42483607867721	1.3551724137931\\
2.43643354819682	1.35862068965517\\
2.44798818663329	1.36206896551724\\
2.45950031164808	1.36551724137931\\
2.47097025983314	1.36896551724138\\
2.48239838452703	1.37241379310345\\
2.49378505380475	1.37586206896552\\
2.50513064862927	1.37931034482759\\
2.51643556115347	1.38275862068966\\
2.52770019316178	1.38620689655172\\
2.53892495464151	1.38965517241379\\
2.55011026247428	1.39310344827586\\
2.56125653923894	1.39655172413793\\
2.57236421211736	1.4\\
};
\addlegendentry{data6}

\addplot [color=black]
  table[row sep=crcr]{%
-2.23331129543969	1.3\\
-2.2456099189327	1.30344827586207\\
-2.25786587195479	1.30689655172414\\
-2.27007867670025	1.31034482758621\\
-2.28224794427973	1.31379310344828\\
-2.2943733678611	1.31724137931034\\
-2.3064547161917	1.32068965517241\\
-2.31849182749742	1.32413793103448\\
-2.33048460375079	1.32758620689655\\
-2.34243300529783	1.33103448275862\\
-2.35433704583153	1.33448275862069\\
-2.36619678769857	1.33793103448276\\
-2.37801233752467	1.34137931034483\\
-2.38978384214373	1.3448275862069\\
-2.40151148481505	1.34827586206897\\
-2.41319548171356	1.35172413793103\\
-2.42483607867721	1.3551724137931\\
-2.43643354819682	1.35862068965517\\
-2.44798818663329	1.36206896551724\\
-2.45950031164808	1.36551724137931\\
-2.47097025983314	1.36896551724138\\
-2.48239838452703	1.37241379310345\\
-2.49378505380475	1.37586206896552\\
-2.50513064862927	1.37931034482759\\
-2.51643556115347	1.38275862068966\\
-2.52770019316178	1.38620689655172\\
-2.53892495464151	1.38965517241379\\
-2.55011026247428	1.39310344827586\\
-2.56125653923894	1.39655172413793\\
-2.57236421211736	1.4\\
};
\addlegendentry{data7}

\addplot [color=black]
  table[row sep=crcr]{%
0.86	1.326\\
0.929412739415687	1.32758620689655\\
0.990545483281801	1.33103448275862\\
1.02963393518102	1.33448275862069\\
1.06035711042955	1.33793103448276\\
1.08630175112185	1.34137931034483\\
1.10905677557982	1.3448275862069\\
1.12949231819793	1.34827586206897\\
1.14814628364591	1.35172413793103\\
1.16537872377472	1.3551724137931\\
1.18144465376449	1.35862068965517\\
1.19653250228011	1.36206896551724\\
1.21078615728211	1.36551724137931\\
1.22431842821669	1.36896551724138\\
1.23721968726884	1.37241379310345\\
1.24956364576018	1.37586206896552\\
1.26141134771563	1.37931034482759\\
1.27281401043963	1.38275862068966\\
1.28381509472055	1.38620689655172\\
1.29445184569351	1.38965517241379\\
1.30475646102415	1.39310344827586\\
1.31475699105245	1.39655172413793\\
1.32447804248352	1.4\\
};
\addlegendentry{data8}

\addplot [color=black]
  table[row sep=crcr]{%
0.86	1.326\\
0.784566539661727	1.32758620689655\\
0.715269574094674	1.33103448275862\\
0.667975084090887	1.33448275862069\\
0.628995965529202	1.33793103448276\\
0.594736276908402	1.34137931034483\\
0.563596599650933	1.3448275862069\\
0.534694761359401	1.34827586206897\\
0.507478984057304	1.35172413793103\\
0.481573129809723	1.3551724137931\\
0.456703400280504	1.35862068965517\\
0.432659257203021	1.36206896551724\\
0.409270546630737	1.36551724137931\\
0.386392923960937	1.36896551724138\\
0.363897691917939	1.37241379310345\\
0.341663899575039	1.37586206896552\\
0.319571303553098	1.37931034482759\\
0.297493028737222	1.38275862068966\\
0.275286607895773	1.38620689655172\\
0.252781414359191	1.38965517241379\\
0.229758858139499	1.39310344827586\\
0.205917711018508	1.39655172413793\\
0.180806227936438	1.4\\
};
\addlegendentry{data9}

\addplot [color=black]
  table[row sep=crcr]{%
-0.86	1.326\\
-0.929412739415687	1.32758620689655\\
-0.990545483281801	1.33103448275862\\
-1.02963393518102	1.33448275862069\\
-1.06035711042955	1.33793103448276\\
-1.08630175112185	1.34137931034483\\
-1.10905677557982	1.3448275862069\\
-1.12949231819793	1.34827586206897\\
-1.14814628364591	1.35172413793103\\
-1.16537872377472	1.3551724137931\\
-1.18144465376449	1.35862068965517\\
-1.19653250228011	1.36206896551724\\
-1.21078615728211	1.36551724137931\\
-1.22431842821669	1.36896551724138\\
-1.23721968726884	1.37241379310345\\
-1.24956364576018	1.37586206896552\\
-1.26141134771563	1.37931034482759\\
-1.27281401043963	1.38275862068966\\
-1.28381509472055	1.38620689655172\\
-1.29445184569351	1.38965517241379\\
-1.30475646102415	1.39310344827586\\
-1.31475699105245	1.39655172413793\\
-1.32447804248352	1.4\\
};
\addlegendentry{data10}

\addplot [color=mycolor1, draw=none, mark=o, mark options={solid, mycolor1}]
  table[row sep=crcr]{%
-0.379609792565303	1.37\\
1.2282514273249	1.37\\
1.36422627993204	1.37\\
2.47440307222837	1.37\\
3.10978768641905	1.37\\
};
\addlegendentry{data11}

\addplot [color=mycolor2, draw=none, mark=triangle, mark options={solid, mycolor2}]
  table[row sep=crcr]{%
0.379609792565303	1.37\\
-1.2282514273249	1.37\\
-1.36422627993204	1.37\\
-2.47440307222837	1.37\\
-3.10978768641905	1.37\\
};
\addlegendentry{data12}

\end{axis}
\end{tikzpicture}%
